Differentiable Particles for General-Purpose Deformable Object Manipulation

Deformable object manipulation is a long-standing challenge in robotics. While existing approaches often focus narrowly on a specific type of object, we seek a general-purpose algorithm, capable of manipulating many different types of objects: beans, rope, cloth, liquid, . . . . One key difficulty is a suitable representation, rich enough to capture object shape, dynamics for manipulation and yet simple enough to be acquired effectively from sensor data. Specifically, we propose Differentiable Particles (DiPac), a new algorithm for deformable object manipulation. DiPac represents a deformable object as a set of particles and uses a differentiable particle dynamics simulator to reason about robot manipulation. To find the best manipulation action, DiPac combines learning, planning, and trajectory optimization through differentiable trajectory tree optimization. Differentiable dynamics provides significant benefits and enable DiPac to (i) estimate the dynamics parameters efficiently, thereby narrowing the sim-to-real gap, and (ii) choose the best action by backpropagating the gradient along sampled trajectories. Both simulation and real-robot experiments show promising results. DiPac handles a variety of object types. By combining planning and learning, DiPac outperforms both pure model-based planning methods and pure data-driven learning methods. In addition, DiPac is robust and adapts to changes in dynamics, thereby enabling the transfer of an expert policy from one object to another with different physical properties, e.g., from a rigid rod to a deformable rope.

==> sections/transferability.tex <==
\subsection{Transferability}
\label{sec:transferability}

In this section, we define the policy transferability between different environments. To understand the transferability, we first ask two key questions: 1) what is different between the source and target domain? 2) what is transferred/common, between the source and target domain?

\begin{definition}
We define a \textbf{task} as MDP tuple $m = (S, A, T, R)$ with state space $S$, action space $A$, transition function $T$ and reward function $R$.
\end{definition}


\begin{definition}
We define a \textbf{transferability} $c_\theta(m,\hat{m})$ as $\frac{\E[R(\tau_{\hat{m}})]}{\E[R(\tau_m)]} $, respecting to a policy $\pi_\theta$ from source task $m$ to target task $\hat{m}$, given $S_{\hat{m}} \subseteq S_m$, $A_{\hat{m}} \subseteq A_m$,   $R_{\hat{m}} = R_m$ and $T \ne \hat{T}$.
\end{definition}

The transferability is only defined with conditions $S_{\hat{m}} \subseteq S_m$, $A_{\hat{m}} \subseteq A_m$ and  $R_{\hat{m}} = R_m$, otherwise the transferability is undefined and not meaningful. With the understanding of the transferability $c_\theta(m,\hat{m})$, we can intentionally increase the state space of the source domain to facilitate the transfer. If we write the hard constraints in Lagrange form:
\begin{align}
    \argmax_{m,\hat{m}, \theta} \; c_\theta(m,\hat{m})
   &= \frac{\E[R(\tau_{\hat{m}})]}{\E[R(\tau_m)]} + \lambda ( \frac{|S_{\hat{m}} \cap S_m|}{|S_{\hat{m}}|} - 1) \nonumber \\
   &+ \beta ( \frac{|A_{\hat{m}} \cap A_m|}{|A_{\hat{m}}|} - 1)
   \label{eq:tf1}
\end{align}



In fact, both domain randomization and domain adaptation are the special cases of our framework $S_{\hat{m}} \subseteq S_m$. Domain randomization explicitly increase source domain $S_m$ and domain adaptation reduces the target domain $S_{\hat{m}}$ to help with the transfer. Within our formulation, we can foresee the the failure cases of domain randomization and domain adaption in scenarios, where the transition functions $T_\varphi$ and $\hat{T}_\varphi$ are conflicting with each other.

\textbf{Practical Approximation}. In the task of deformable objects, the state space and action space can be extremely large and are intractable to iterate all of them. To practically measure the transferability between source task $m$ and target task $\hat{m}$ respect to the policy $\pi_\theta$, we sample $S_{m,\theta} \subset \tau_m$ in task $m$ and $\hat{S}_{m,\theta} \subset \hat{\tau}_m$ in task $\hat{m}$ to approximate the transferability score $c_\theta(m,\hat{m})$. Alternative soft unidirectional Chamfer constraint on each state:

\begin{align}
     \argmax_{m,\hat{m}, \theta} \; c_\theta(m,\hat{m}) &= \frac{\E[R(\tau_{\hat{m}})]}{\E[R(\tau_m)]} + \lambda \sum_{\hat{s} \in S_{\hat{m}}} \min_{s \in S_m} ||\hat{s} - s||_2^2 \nonumber \\
     &+ \beta \sum_{\hat{a} \in A_{\hat{m}}} \min_{a \in A_m} ||\hat{a} - a||_2^2 \; \;
\end{align}


\textbf{Potential Usage}. We have the transferability defined in \eqref{eq:tf1}, and it begs to the question: how can we use the  formulation to improve the transferability? There are many options: 1) \textbf{Domain randomization}. We can increase $S_m$ to reduce the state gap. 2) \textbf{Domain adaptation}. 3) \textbf{Policy Adaptation}. We can better construct $m$ to be close to $\hat{m}$, and then better construct $\pi_\theta$ to perform well in $m$. It then begs to the idea: instead of training $\pi_\theta$ in $m$ that can be far from $\hat{m}$, we should construct $\hat{m}'$ that is close to $\hat{m}$ and then train $\pi_\theta$ in $\hat{m}'$. For example, if $\pi_\theta$ is IL agent, we should collect new demonstrations in simulation under the newly estimated $\hat{m}'$ to train $\pi_\theta$.




==> tables/real_robot_bean.tex <==
\begin{table}[t]
\centering
\caption{\small Real Robot Bean Sweeping Results}
% \fontsize{8}{8}\selectfont


\begin{tabular}{lccc}
\toprule
Method              &  Count      & Avg Steps & Avg Steps Std         \\ 
\midrule

Transporter*        &    6/10         &   6.60 & 2.65  \\
CEM-MPC   &     & & \\
\anameDipac w random init policy (ours)       &     10/10        &    6.40  &    1.85       \\
\anameDipac (ours)       &    10/10         &      6.50 &  2.81        \\

\bottomrule
\end{tabular}

\label{table:bean_results}
\end{table}


==> tables/real_robot_rope.tex <==
\begin{table}[t]
\centering
\caption{\small Real Robot Rope Pushing Results}
% \fontsize{8}{8}\selectfont

\begin{tabular}{lccc}
\toprule
Method              &  Count      & Avg Steps & Steps Std         \\ 
\midrule

Transporter*        &     4/10        &   9.75 & 3.70  \\
CEM-MPC    &      0/10     &  - & -\\
\anameDipac w random init policy (ours)       &     7/10        &    13.29  &    6.71       \\
\anameDipac (ours)       &     9/10        &    12.78  &    6.63       \\

\bottomrule
\end{tabular}

\label{table:rope_results}
\end{table}

==> tables/real_robot_rope_ablation.tex <==
\begin{table}[t]
\centering
\vspace{-10pt}
\caption{\small Ablations on Real Robot Rope Pushing Task}
% \fontsize{8}{8}\selectfont

\begin{tabular}{lccc}
\toprule
Method              &  Count      & Avg Steps & Steps Std         \\ 
\midrule

\anameDipac (ours)       &     9/10        &    12.78  &    6.63       \\
\anameDipac w/o diff optimization       &   3/10          &  17.00    &     9.90      \\
\anameDipac w/o exploration       &   6/10          &  15.00    &     7.16      \\
\anameDipac w/o obs adaptation       &   4/10          &  9.50    &     3.50      \\
\anameDipac w/o diff SI       &   9/15          &   19.11   &   4.25        \\

\bottomrule
\end{tabular}

\label{table:ablation_results}
\end{table}
